From the Densest Clusters to the Emptiest Voids: No Evidence For Environmental Effects on the Galaxy Size-Mass Relation at Low Redshift

We present a comprehensive study of the galaxy size-stellar mass relation (SMR) at low redshift (z <= 0.125), using a large spectroscopic sample from the SDSS-DR13 survey. Our goal is to investigate how environment affects galaxy structural properties across multiple spatial scales. Galaxies are classified by specific star formation rate, optical color, and bulge-to-total light ratio, allowing us to disentangle environmental effects from intrinsic galaxy properties. We examine the SMR in three contexts: (1) comparing galaxy sizes in two extreme environments-dense clusters versus cosmic voids; (2) analyzing cluster galaxies across a range of cluster masses; and (3) studying member galaxies located in different cluster regions, from the core to the infall zone. In all three cases, we find no significant dependence of the SMR on environment at fixed stellar mass and galaxy type. Cluster and void galaxies follow consistent SMR trends, and no measurable variation is observed with cluster mass or cluster-centric distance. We also confirm that early-type galaxies exhibit steeper SMR slopes than late types. Notably, this consistent lack of environmental dependence on the SMR persists even when accounting for the differing galaxy number densities in voids, supporting the universality of this SMR scaling relation across diverse environments.

==> name.tex <==
\begin{table*}
\centering
\caption{Summary of studies investigating the environmental dependence of the galaxy size--mass relation.
%The table lists selected previous studies, their redshift range ($z$), the method used to define environment, and the physical environmental scales probed in each study. 
LS= large-scale, SS = small-scale, Cls = cluster, F = field, Sat= satellite, Cen=central, ET= early-type, SF=star-forming, Q= quiescent, E= elliptical.}
\label{tab:env}
\begin{tabular}{lcccccc}
\hline
Study & $z$ range & quality & Environment & Scale & $\log{M_\star}$~[\hmm] & comment\\
\hline
\multicolumn{7}{c}{Environmental Independence} \\
\hline
This work                   & 0.01--0.125   & spec     & Cls/F          & LS/SS &$\geq$10.00&$f(M_h)$ \& $f(R_p)$\\
\cite{Strazzullo2023}       & 1.40--1.70   & phot/spec & Cls/F          & LS    & $\geq$$10.54$&\\
\cite{Afanasiev2023}        & 1.40--2.80   & spec  & Cls/F                 & LS & 9.29-10.19 &\\
\cite{Zhang2019}            & 0.01--0.20   &           & den contrast   & LS    &&\\
\cite{Mosleh2018}           & 0.01--0.05   & spec      & Cls/F          & LS    & $\geq$9.69& Q \\
\cite{Tran17}               & $\sim 2.00$  & spec      & Cls/F          & LS    & $\geq$8.69& SF\\
\cite{Saracco2017}          & 1.20--1.40   & phot/spec & Cls/F          & LS    & $\geq$9.20 & E\\
\cite{Kelkar2015}           & 0.40--0.80   & phot/spec & Cls/F          & LS    &$\geq$9.89&\\
\cite{Shankar2014}          & 0.05--0.20   &  spec     & Cls/F          & LS    &$\geq$10.93& ET\\
\cite{Newman2014}           & $\sim 1.80$  &          spec & Cls/F          & LS    &$\geq$10.19& Q\\
\cite{Huertas-Company2013a} & 0.20--1.00   & phot/spec & Cls/F          & LS    &$\geq$10.19& ET\\
\cite{Huertas13a}           & $<0.09$      &    spec   & Cls/F          & LS/SS &$\geq$10.19 &ET, $f(M_h)$ \& $f(R_p)$\\
\cite{Rettura2010}          & $\sim 1.20$  &           & Cls/F          & SS    &&\\
\cite{Maltby2010}           & $\sim 0.17$  &   phot    & Cls/F          & LS    &$\geq$9.69&\\
\cite{Guo2009}              & 0.04--0.07   &    spec       & Cen/Sat        & SS   &$\geq$10.0&\\
%\cite{Cimatti2008}          & 1.40--2.00   &           & den contrast   & SS    &&\\
\hline
\multicolumn{7}{c} {Environmental Dependence} \\
\hline
\cite{Perez2025}            & 0.01--0.05   & spec & Cls/F                 & LS& 8.19-10.69& \\
\cite{Chamba24}             & $<0.02$      & spec & Cls/F                 & LS & 4.69-10.69& \\
\cite{Ghosh24}              & 0.30--0.70   & phot & den contrast   & LS & $\geq$$8.55$ &\\
\cite{Afanasiev2023}        & 1.40--2.80   & spec  & Cls/F                 & LS & $\geq$10.19 &\\
\cite{Xu2023}               & 2.49--2.52   &  & Cls/F                 & LS &$\geq$10.19&SF\\
\cite{Tan2022}              & 0.25--0.60   &  & den contrast   & LS &\\
\cite{Noordeh21}            & 1.90--2.10   &  & Cls/F                 & LS &\\
\cite{Matharu2021}          & 0.86--1.34   &  & Cls/F                 & LS &\\
\cite{Matharu2020}          & 0.86--1.34   &  & Cls/F                 & LS &\\
\cite{Zhang2019}            & 0.01--0.20   &  & den contrast   & LS &\\
\cite{Demers2019}           & 0.01--0.06   &  & Cls/F                 & LS &\\
\cite{Matharu19}            & 0.86--1.34   &  & Cls/F                 & LS &\\
\cite{Huang2018}            & 0.30--0.50   &  & den contrast   & LS &\\
\cite{Kuchner2017}          & 0.44         &  & Cls/F                 & LS &\\
\cite{Yoon2017}             & 0.01--0.15   &  & den contrast   & LS &\\
\cite{Morishita2017}        & 0.20--0.70   &  & Cls/F                 & SS &\\
\cite{Cebrian2014}          & 0.01--0.12   &  & den contrast   & LS &\\
\cite{Delaye2014}           & 0.80--1.50   &  & Cls/F                 & SS &\\
\cite{Poggianti13}          & 0.03--0.11   &  & Cls/F                 & SS &\\
\cite{Lani2013}             & 0.50--2.00   &  & den contrast   & SS &\\
\cite{Capellari2013}        & 0.01--0.02   &  & Cls/F                 & LS &\\
\cite{Lorenzo2013}          & 0.01--0.05   &  & den contrast   & LS &\\
\cite{Strazzullo13}         & $\sim 2.00$  &  & Cls/F                 & SS &\\
\cite{Raichoor2012}         & 0.92--1.40   &  & den contrast    & SS &\\
\cite{Cooper2012}           & 0.40--1.20   &  & den contrast   & SS &\\
\cite{Papovich2012}         & 1.5          &  & Cls/F                 & LS &\\
\cite{delaye2012}           & 0.80--1.15   &  & Cls/F                 & SS &\\
\cite{Valentinzzi2010}      & 0.04--0.07   &  & den contrast   & LS &\\
\cite{Weinmann2009}         & 0.01--0.20   &  & Sat/Cen         & LS &\\
\hline
\end{tabular}
\end{table*}


\begin{table*}
\centering
\caption{Summary of studies investigating the environmental dependence of the galaxy size--mass relation.
LS = large-scale, SS = small-scale, Cls = cluster, F = field, Sat = satellite, Cen = central, ET = early-type, SF = star-forming, Q = quiescent, E = elliptical. The ``Trend'' column indicates the reported direction of the environmental dependence when a study finds a significant effect.}
\label{tab:env}
\begin{tabular}{lcccccc}
\hline
Study & $z$ range & quality & Environment & Scale & $\log{M_\star}$~[\hmm] & Trend \\
\hline
\hline
\multicolumn{7}{c}{Environmental Independence} \\
\hline
This work                   & 0.01--0.125   & spec      & Cls/F        & LS & $\geq$10.00 & none \\
\cite{Afanasiev2023}        & 1.40--2.80    & spec      & Cls/F        & LS    & 9.30--10.20 & none \\
\cite{Zhang2019}            & 0.01--0.12    &    spec       &   den contrast & LS    &       $\geq$8.70      & negligible \\
\cite{Mosleh2018}           & 0.01--0.05    & spec      & Cls/F        & LS    & $\geq$9.70  & none \\
\cite{Tran17}               & $\sim 2.00$   & spec      & Cls/F        & LS    & $\geq$8.70  & none \\
\cite{Shankar2014}          & 0.05--0.20    & spec      & Cls/F        & LS    & $\geq$10.90 & none \\
\cite{Newman2014}           & $\sim 1.80$   & spec      & Cls/F        & LS    & $\geq$10.20 & none \\
\cite{Huertas13a}           & $<0.09$       & spec      & Cls/F        & LS & $\geq$10.20 & none \\

\cite{Strazzullo2023}       & 1.40--1.70    & phot/spec & Cls/F        & LS    & $\geq$10.50 & none \\
\cite{Morishita2017}        & 0.20--0.70    &     phot/spec      & Cls/F        & LS    &         $\geq$7.50  & negligible \\
\cite{Saracco2017}          & 1.20--1.40    & phot/spec & Cls/F        & LS    & $\geq$9.20  & none \\
\cite{Kelkar2015}           & 0.40--0.80    & phot/spec & Cls/F        & LS    & $\geq$9.90  & none \\
\cite{Rettura2010}          & $\sim 1.20$   &   phot/spec        & Cls/F        & LS    &   $\geq$10.40          & none \\
\cite{Huertas-Company2013a} & 0.20--1.00    & phot/spec & Cls/F        & LS    & $\geq$10.20 & none \\
\cite{Maltby2010}           & $\sim 0.17$   & phot      & Cls/F        & LS    & $\geq$9.70  & none \\
This work                   & 0.01--0.125   & spec      & $f(R_p)$ \& $f(M_h)$        & SS & $\geq$10.00 & none \\
\cite{Huertas13a}           & $<0.09$       & spec      &$f(R_p)$ \& $f(M_h)$        & SS & $\geq$10.20 & none \\
%\cite{Guo2009}              & 0.04--0.07    & spec      & Cen/Sat      & SS    & $\geq$10.0  & none \\
\hline
\hline
\multicolumn{7}{c}{Environmental Dependence} \\
\hline
\cite{Perez2025}            & 0.01--0.05    & spec      & Cls/F        & LS    & $\geq$8.20 & $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\
\cite{Afanasiev2023}        & 1.40--2.80    & spec      & Cls/F        & LS    & $\geq$10.20 & $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\
%\cite{Tan2022}              & 0.25--0.60    &           & den contrast & LS    &             &  \\
\cite{Noordeh21}            & 1.90--2.10    &  spec         & Cls/F        & LS    &       $\geq$10.00      & $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\
%\cite{Huang2018}            & 0.30--0.50    &           & den contrast & LS    &             &  \\
%\cite{Kuchner2017}          & 0.44          & phot/spec          & Cls/F        & LS    &             &  \\
\cite{Yoon2017}             & 0.01--0.15    &      spec     & den contrast & LS    &     $\geq$10.70        &  $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\
\cite{delaye2014}           & 0.80--1.50    &     spec      & Cls/F        & LS    &     $\geq$10.20        &  $R_\mathrm{{CLs}}>R_\mathrm{F}$  \\
%\cite{Poggianti13}          & 0.03--0.11    &           & Cls/F        & SS    &             &  \\
%\cite{Capellari2013}        & 0.01--0.02    &           & Cls/F        & LS    &         $\geq$9.50    &  \\
%\cite{Lorenzo2013}          & 0.01--0.05    &           & den contrast & LS    &             &  \\
\cite{Cooper2012}           & 0.40--1.20    &   spec        & den contrast & LS    &     $\geq$10.00        &  $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\

\cite{Strazzullo13}         & $\sim 2.00$   &    phot/spec       & Cls/F        & LS    &      $\geq$10.00        &   $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\
\cite{Ghosh24}              & 0.30--0.70    & phot      & den contrast & LS    & $\geq$8.60  & $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\
\cite{Lani2013}             & 0.50--2.00    &   phot        & den contrast & LS    &          $\geq$10.00   &  $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\
\cite{Papovich2012}         & 1.5           &    phot       & Cls/F        & LS    &      $\geq$10.20        &  $R_\mathrm{{CLs}}>R_\mathrm{F}$ \\

\cite{Chamba24}             & $<0.02$       & spec      & Cls/F        & LS    & $\geq$4.70 & $R_\mathrm{{CLs}}<R_\mathrm{F}$ \\
\cite{Xu2023}               & 2.49--2.52    &  spec         & Cls/F        & LS    & $\geq$10.20 & $R_\mathrm{{CLs}}<R_\mathrm{F}$ \\
\cite{Matharu2021}          & 0.86--1.34    &    spec       & Cls/F        & LS    &        $\geq$9.30     & $R_\mathrm{{CLs}}<R_\mathrm{F}$ \\
\cite{Demers2019}           & 0.01--0.06    & spec          & Cls/F        & LS    &    9.50-9.90     & $R_\mathrm{{CLs}}<R_\mathrm{F}$ \\
\cite{Matharu19}            & 0.86--1.34    &   spec        & Cls/F        & LS    &    $\geq$9.60 &   $R_\mathrm{{CLs}}<R_\mathrm{F}$      \\
\cite{Cebrian2014}          & 0.01--0.12    &    spec       & den contrast & LS    &        $\geq$10.00     & $R_\mathrm{{CLs}}<R_\mathrm{F}$ \\
%\cite{Matharu2020}          & 0.86--1.34    &           & Cls/F        & LS    &             &  \\
%\cite{Zhang2019}            & 0.01--0.20    &     spec      & Cls/F & LS    &    8.70-10.20         & $R_\mathrm{{Cls}}<R_\mathrm{F}$  \\


\hline
\end{tabular}
\end{table*}


%\textcolor{violet}{Across several investigations, numerous studies have explored the impact of environment on the galaxy SMR. Yet their findings remain inconsistent, While some reported a significant dependence on environment. Many attempts found a little to no environmental effects. For better insight to the source of all these discrepancies, we compile the main outcome results of more than 40 studies, investigated the environmental dependence of the SMR. Table~\ref{tab:env} summarizes key aspects of these works, including the reference, redshift range and whether or not an environmental effect was declared. To be more clarifying and objective, we limit table ~\ref{tab:env} to  the most triggered and essential findings of the previous studies.} \textcolor{red}{be careful: the no of the corresponding table in this paragraph is mismatching with the no of table below.here we have table 4 while below the no of table is 3 !!}



%While each of the above factors may influence the outcome to some extent, none of them individually accounts for the variation in \underline{reported} \textcolor{violet}{the testified} environmental effects. Instead, the\textcolor{violet}{se} discrepancies \underline{likely arise} \textcolor{violet}{are strongly recommended to be emerged} from a combination of \textcolor{violet}{several} factors, including how stellar masses and galaxy sizes are measured, whether redshifts are photometric or spectroscopic, how galaxies are classified, the definition of environment, the redshift range probed, and the number of galaxies included in the sample. In particular, studies with \underline{small samples} \textcolor{violet}{a small sample of galaxies} may suffer from limited statistical power, while larger samples often rely on photometric redshifts and mass estimates, which introduce their own uncertainties. The interplay among these elements makes it difficult to isolate a dominant source of disagreement. This suggests that conclusions about the presence or absence of environmental effects on the size mass relation must be interpreted within the broader context of each study’s design, assumptions, and data quality.

%Several aspects of our methodology \underline{give us confidence} \textcolor{violet}{confirms the reliability of our findings}. Our analysis is built on a large and statistically powerful spectroscopic sample drawn from the SDSS, allowing for precise measurements and robust conclusions. To ensure a clear environmental contrast, we adopt extreme definitions for both cluster and field galaxies: cluster members are selected using the GalWCat19 spectroscopic catalog. \textcolor{violet}{Field galaxies are drawn from the lowest-density regions, outside any known structures, assigning each void with 8 galaxies only}. We exclude sparse data from the main sample that could bias the results due to low-number statistics. For structural measurements, we rely on a recent, high-quality galaxy size catalog with improved measurement efficiency and consistency. Stellar masses are taken from the MPA/JHU catalog, which \underline{derives} \textcolor{violet}{were derived directly from galaxies spectra}, \underline{ensuring} \textcolor{violet}{assuring the} reliability. Together, these methodological choices minimize uncertainties and observational biases, giving us high confidence in the robustness of our result: that the size mass relation does not show a significant dependence on environment when controlling for galaxy type and stellar mass.


%\item Stellar mass measurement: We find no consistent correlation between the reported  environmental dependence and the method used to derive stellar masses. 
%{\bf{To verify this, we used photometrically derived stellar masses provided by the Granada group \footnote{\url{https://www.sdss4.org/dr17/spectro/galaxy_granada/}},}} calculated using the publicly available Flexible Stellar Population Synthesis code \citep{Conroy09}, instead of spectroscopic estimates, and again found no evidence of an environmental effect. The results, omitted here for brevity, align with our main findings.

%\item Galaxy size definition:
%The choice of size definition also does not appear to explain the discrepant results. Previous studies have used a variety of structural measures, including effective radius, semi-major axis, and other size estimators. Yet both positive and null environmental effects are reported across these different definitions, suggesting that the size metric itself is unlikely to be the dominant source of disagreement.
